Multi-layered Network Exploration via Random Walks: From Offline Optimization to Online Learning

Multi-layered network exploration (MuLaNE) problem is an important problem abstracted from many applications. In MuLaNE, there are multiple network layers where each node has an importance weight and each layer is explored by a random walk. The MuLaNE task is to allocate total random walk budget $B$ into each network layer so that the total weights of the unique nodes visited by random walks are maximized. We systematically study this problem from offline optimization to online learning. For the offline optimization setting where the network structure and node weights are known, we provide greedy based constant-ratio approximation algorithms for overlapping networks, and greedy or dynamic-programming based optimal solutions for non-overlapping networks. For the online learning setting, neither the network structure nor the node weights are known initially. We adapt the combinatorial multi-armed bandit framework and design algorithms to learn random walk related parameters and node weights while optimizing the budget allocation in multiple rounds, and prove that they achieve logarithmic regret bounds. Finally, we conduct experiments on a real-world social network dataset to validate our theoretical results.

==> MuLaNE Camera Ready ICML2021/content/acknowledgement.tex <==
\section{Acknowledgement}
The work of John C.S. Lui was supported in part by the GRF 14200420.

==> MuLaNE Camera Ready ICML2021/content/conclusion.tex <==
%%\vspace{-7pt}
\section{Conclusions and Future Work}\label{sec: conclusion}
%%\vspace{-7pt}
This paper formulates the multi-layered network exploration via random walks (\mulane) as a budget allocation problem, requiring that the total weights of distinct nodes visited on the multi-layered network is maximized.
% We systematically study the \mulane{} problem from offline optimization to online learning for both overlapping and non-overlapping networks.
% For the offline setting, we propose offline algorithms which achieve a constant ratio approximation for the overlapping case and the optimal solution for the non-overlapping case.
For the offline setting, we propose four algorithms for \mulane{} according to the specification of multi-layered network (overlapping or non-overlapping) and starting distributions (arbitrary or stationary), each of which has a provable guarantee on approximation factors and running time.
We further study the online setting where network structure and the node weights are not known a priori.
We propose the CUCB-MAX algorithm for overlapping \mulane{} and the CUCB-MG algorithm for the non-overlapping case, both of which are bounded by a $O(\log T)$ (approximate) regret.
Finally, we conduct experiments on a social network dataset to show the empirical performance of our algorithms.

There are many compelling directions for the future study.
For example, it would be interesting to extend our problem where the decision maker can jointly optimize the starting distribution and the budget allocation.
One could also study the adaptive \mulane{} by using the feedback from
the exploration results of the previous steps to determine the exploration strategy for future steps.



==> MuLaNE Camera Ready ICML2021/content/experiments.tex <==
%%\vspace{-6pt}
\section{Experiments}\label{sec: experiments}
%%\vspace{-3pt}
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/offline/fftwyt_uniform_overlapping_smaller_2500_3000_05.pdf}
		\caption{Offline, overlapping.}
		\label{fig: offline over fix}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/offline/fftwyt_uniform_non-overlapping_smaller_2500_3000_05.pdf}
		\caption{Offline, non-overlapping.}
		\label{fig: offline non over fix}
	\end{subfigure}
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/overlapping/new2_fftwyt_ci_overlapping_uniform_3000.pdf}
		\caption{Online, overlapping.}
		\label{fig: online over fix 3000}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/non-overlapping/icml_fftwyt_ci_non_overlapping_uniform_3000.pdf}
		\caption{Online, non-overlapping.}
		\label{fig: online non over fix 3000}
	\end{subfigure}
	%%\vspace{-10pt}
	\caption{Above: total weights of unique nodes visited for offline algorithms. Below: regret for online algorithms when $B=3000$.
	}\label{fig: offline algorithms}
\end{figure}

\begin{table}
\centering
%%\vspace{-5pt}
\caption{Statistics for FF-TW-YT network}
\label{tab: FF-TW-YT}
\begin{minipage}{0.90\columnwidth}
\begin{tabular}{cccc}
    \toprule
        Layer&FriendFeed & Twitter & YouTube  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     \# of vertices & 5,540 & 5,702 & 663 \\
     \# of edges & 31,921 & 42,327 & 614\\
     %FriendFeed (FF) & 5,540 & 31,921 \\
     %Twitter (TW) & 5,702 & 42,327 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
\end{minipage}
\end{table}

\begin{table*}[h]
\caption{Running time (seconds) for offline and online algorithms.}
% \vspace{-6pt}
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \begin{minipage}{0.90\columnwidth}
        \begin{tabular}{cccccc}
    \toprule
     & B=2.6k & B=2.8k & B=3.0k  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     BEG & 0.274 & 0.316 & 0.363 \\
    %  MG & 0.028  & 0.031 &  0.033\\
     BEGE & 34.37  & 45.51 &  59.20 \\
     OPT & 91.16 & 98.42 &  105.63 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
\end{minipage}
       \caption{Running time of offline algorithms for the overlapping case with different budgets B.}
       \label{tab:offline, over}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \begin{tabular}{cccc}
    \toprule
      & B=2.6k & B=2.8k & B=3.0k  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     DP & 0.038  & 0.044 &  0.050 \\
     MG & 0.008  & 0.009 &0.010\\
     OPT & 70.10  & 75.78 & 81.11 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
        \caption{Running time of offline algorithms for the non-overlapping case with different budgets B.}
        \label{tab:offline, non-over}
     \end{subtable}
     \hfill
         \begin{subtable}[h]{0.3\textwidth}
        \centering
        \begin{tabular}{ccc}
    \toprule
     Overlapping? & \checkmark  & $\times$  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     BEG & 1.22  & NA \\
     BEGE & 60.03  & NA\\
     DP  & NA  & 0.86  \\
     OPT & 107.33 & 82.01 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
        \caption{Per-round running time for CUCB-MAX (or CUCB-MG) with different oracles when B=3.0k.
%        	, NA means not applicable.
        }
        \label{tab:online}
     \end{subtable}
     \vspace{-10pt}
     \label{tab:runing time}
\end{table*}

\textbf{Dataset and settings.} We conduct experiments on a real-world multi-layered network FF-TW-YT, which contains $m=3$ layers representing users' social connections in FriendFeed (FF), Twitter (TW) and YouTube (YT)~\cite{dickison2016multilayer}.
% This multi-layered network is built upon the FF network, and the TW and YT layers are generated by exploiting the feature of FriendFeed as a social media aggregator.
In total, FF-TW-YT has $6,407$ distinct vertices representing users and $74,836$ directed edges representing connections (``who follows whom") among users.
The statistics for each layer is summarized in Table~\ref{tab: FF-TW-YT}.
% \textbf{Experimental settings.}
We transform the FF-TW-YT network $\cG(\cV,\cE)$ into a symmetric directed
network (by adding a new edge $(v,u)$ if $(u,v)\in \cE$ but $(v,u) \notin \cE$) because a user can be visited via her followers or followees.
Each edge weight is set to be $1$ and the node weights are set to be $\sigma_u\in\{0,0.5,1\}$ uniformly at random. 
Each random walker always starts from the smallest node-id in each layer and we set constraints $c_i$ equal to the total budget $B$. 
Note that in order to test the non-overlapping case, we use the same network but relabel node-ids so that they do not overlap between different layers.
To handle the randomness, we repeat $10,000$ times and present the averaged total weights of unique nodes visited for offline optimization.
We calculate the regret by comparing with the \textit{optimal} solution, which is stronger than comparing with $(1-e^{-\eta},1)$-approximate solution as defined in Eq.~(\ref{eq: alpha beta regret}).
We average over 200 independent experiments to provide the mean regret with 95\% confidence interval.
To evaluate the computational efficiency, we also present the running time for both offline and online algorithms in Table~\ref{tab:runing time}.

% \vspace{-2pt}
\noindent\textbf{Algorithms in comparison.}
For the offline setting, we present the results for Alg.~\ref{alg: layer traversal greedy} (denoted as BEG), Alg.~\ref{alg: pure greedy} (denoted as MG), BEG with partial enumeration (denoted as BEGE) and \OnlyInFull{Alg.~\ref{alg: dynamic programming}}\OnlyInShort{the dynamic programming algorithm in the supplementary material} (denoted as DP).
We provide two baselines PROP-S and PROP-W, which allocates the budget proportional to the layer size and proportional to the total weights if we allocate $B/3$ budgets to that layer, respectively.
The optimal solution (denoted as OPT) is also provided by enumerating all possible budget allocations. 
For online settings, we consider CUCB-MAX (Alg.~\ref{alg: over online}) and CUCB-MG \OnlyInFull{(Alg.~\ref{alg: non-over online})}\OnlyInShort{(Sec.~\ref{sec:cucbmg})} algorithms.
We shrink the confidence interval by $\gamma$, i.e., $\rho_{i,u,b} \leftarrow \gamma\rho_{i,u,b}$, to speed up the learning, though our theoretical regret bound requires $\gamma = 1$.
%Note that we no longer have theoretical guarantee when $\gamma < 1$, so the rest can be thought of heuristic algorithms.
For baselines, we consider the EMP algorithm which always allocates according to the empirical mean, and the $\epsilon$-Greedy algorithm which allocates budgets according to empirical mean with probability $1-\epsilon$ and allocates all $B$ budgets to the $i$-th layer with probability $\epsilon/m$.
We also compare with the Thompson sampling (TS) method~\cite{wang2018thompson}, which uses Beta distribution $\text{Beta}(\alpha,\beta)$ (where $\alpha=\beta=1$ initially) as prior distribution for each base arm.

% \vspace{-2pt}
\noindent\textbf{Experimental results.}
We show the results for \mulane{} problems in Figure~\ref{fig: offline algorithms}.
For the offline overlapping case, both BEG and MG outperform
two baselines PROP-W and PROP-S in receiving total weights.
Although not guaranteed by the theory, BEG are empirically close to BEGE and the optimal solution (OPT).
As for the computational efficiency, in Table~\ref{tab:offline, over}, the BEG is at least two orders of magnitude (e.g.,163 times when B=3.0k) faster than BEGE and OPT. 
Combining that the reward of BEG is empirically close to BEGE and the optimal solution, this shows that BEG is empirically better than BEGE and OPT.
For the offline non-overlapping case, the results are similar, but the difference is that we have the theoretical guarantee for the optimality of DP.
% For the online overlapping case, all CUCB-MAX curves grow sub-linearly w.r.t round $T$, due to the fact that our offline oracle achieves near optimal solutions.
% Comparing to two baselines, the CUCB-MAX ($\gamma=1.0$) curve has larger regret because it is relative conservative to theoretically guarantee the regret bound.
% As we decrease $\gamma$, the regret decreases and consistently outperforms baseline algorithms when $\gamma=0.1, 0.05$.
%Although the theoretical guarantee no longer holds when $\gamma < 1$, we have superior empirical performance, which 
For the online setting, all CUCB-MAX/CUCB-MG curves outperform the baselines.
This demonstrates empirically that CUCB-MAX algorithm can effectively learn the unknown parameters while optimizing the objective.
For the computational efficiency of online learning algorithms, since the running time for algorithms with the same oracle is similar, we present the running time for CUCB-MAX with different oracles in Table~\ref{tab:online}.
CUCB-MAX with BEG is 50 times faster than BEGE, which is consistent with our theoretical analysis.
% % For the non-overlapping case, we can observe that the CUCB-MG ($\gamma=1.0$) curve mostly lies between the baseline algorithms.
% % The CUCB-MG algorithm outperforms two baselines when $\gamma$ decreases to $0.5$.
% Interestingly, the regret of CUCB-MG ($\gamma=0.05$) is larger than CUCB-MG ($\gamma=0.01$), which is the opposite for overlapping cases.
% This is because the number of base arms is only $1/|\cV|$ of that for the overlapping case, which makes $\gamma=0.05$ too aggressive for the online learning process.
The results for different budgets $B$ are consistent with $B=3000$, which are included in the \OnlyInFull{Appendix~\ref{appendix: expriment for diff budgets}}\OnlyInShort{supplementary material}.
Results and analysis for stationary starting distributions are also in the\OnlyInFull{ Appendix~\ref{appendix: expriment for stationary distributions}}\OnlyInShort{supplementary material}.



























==> MuLaNE Camera Ready ICML2021/content/introduction.tex <==
%%\vspace{-20pt}
\section{Introduction}
Network exploration is a fundamental paradigm of searching/exploring
in order to discover information and resources available at nodes in a network, 
and random walk is often used as an effective tool for network exploration \cite{lv2002search,gleich2015pagerank,wilder2018maximizing}.
In this paper, we study the multi-layered network exploration via random walks problem, which can model many real-world applications, including resource searching in peer-to-peer (P2P) networks and web surfing in online social networks (OSNs).
% In network data gathering, a data analyst wants to crawl a number of online social networks (OSNs) via application program interfaces (APIs) 
% 	to gather as much information as possible about the nodes in the networks.
% The API returns a random neighbor of a given node, effectively mapping a sequence of iterative API calls to a random walk, which may return
% 	nodes already visited in the past.
% Since the API calls have costs and the analyst has a limited budget, she needs to decide how to allocate her budget among different OSNs
% 	so as to obtain the greatest number of unique nodes visited.
% In online social advertising, an advertiser wants to advertise a new product via different social network platforms through incentives offered to 
% 	 users in order for the users to relay the advertisements to their friends in the social networks.
% The advertiser wants to achieve the similar goal of allocating her budget among different networks so as to maximize the number of people her
% 	advertisement reached.

In P2P networks, a user wants to find resources that are scattered on nodes (i.e. peers) in different P2P networks via some platform-specified strategies.
A commonly used search strategy is based on multiple random walks \cite{lv2002search}.
Since different resources have different importance,
the search quality of different random walkers varies.
Moreover, the resource-search process typically has a life span, i.e., a total time-limit or hop-limit for random walks.
So the user's goal is to decide how to allocate limited budgets to different random walkers to find as many important resources as possible.
Another application is the web surfing, where users want to find information in different OSNs, by looking at posts via others' home-pages~\cite{lerman2006social}.
Once the user arrives at one of his friends' home-pages in a particular OSN, he could find some information and continues to browse the home-pages of his friends' friends, which can be regarded as a random walk process.
Since the user only has a finite duration in web surfing,
the similar question is how to allocate his time in exploring different OSNs so to get the maximum amount of useful information.


% The resource searching application can also find similar counterparts in OSNs, where users primarily rely on the web surfing process to find information along their social ties~\cite{lerman2006social}.
% For example, in micro-blogging websites Twitter, Weibo, etc., a user can view his friends' posts (tweets, likes, retweets, etc.) via their home pages. Once the user arrives at one of his friends' home-page, he can browse posts created by his friends' friends.
% The next home-page that the user will visit depends on the current home-page he is browsing, which can be regarded as a random-walk process.
% Whenever he visits a new home-page, he may find information that may or may not satisfies his interest.
% Nevertheless, users cannot browse an infinite number of home-pages and typically have an implicit time-limit to browse others' homepages.
% The question is how to allocate his time exploring different OSNs to get maximum amount of useful information.

% Social networking service has nowadays become an important
% medium for users to discover information online.
% In OSNs, users primarily rely on a social browsing process to find useful information along their social ties.
% For example, in a micro-blogging website Twitter, a user can view his friends' posts via their home pages. Once the user arrives at one of his friends' home-page, he can apply the same way to browse posts created (liked, retweeted, replied, etc.) by his friends' friends.
% The next home-page that the user will visit depends on the current home-page he is browsing, which can be regarded as a random-walk process.
% Whenever he visits a new home-page, he may find useful information that satisfies his interest.
% Nevertheless, users cannot browse an infinite number of home-pages users in OSNs and typically have an implicit time-limit to browse others' homepages.
% The question is how to allocate his time exploring different OSNs to obtain maximum amount of useful information.           

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/multi-layer/multi-layer_bold.eps}
%         \caption{Overlapping.}
%         \label{fig: over}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/multi-layer/non_over_multi_layered.eps}
%         \caption{Non-overlapping.}
%         \label{fig: non-over}
%     \end{subfigure}
%         \caption{Two types of multi-layered networks.}
%         \label{fig: multi-layered}
% \end{figure}
	
We abstract the above application scenarios as the \textbf{Mu}lti-\textbf{La}yered \textbf{N}etwork \textbf{E}xploration (MuLaNE) problem.
In \mulane, we model the overall network to be explored (e.g., combining different OSNs) as a~multi-layered network $\cG$ that consists of $m$ layers $L_1, ..., L_m$.
Each layer $L_i$ (e.g., a single OSN) is represented by a weighted directed graph $\cG_i(\cV_i,\cE_i,w_i)$,
where $\cV_i$ is the set of nodes to be explored (e.g., users' home-pages with importance weight $\sigma_u$ for $u\in \cV_i$), $\cE_i \subseteq \cV_i \times \cV_i$ is the set of directed edges (e.g., social links), and $w_i$ is the edge weight function on edges $\cE_i$.
Each layer $L_i$ is associated with an explorer (or random walker) $W_i$ and a fixed starting distribution  $\bm{\alpha}_i$ on nodes $\cV_i$.
Explorer $W_i$ starts on a node in $\cG_i$ following the distribution $\bm{\alpha}_i$, and then walks on network $\cG_i$ following outgoing edges with probability proportional to edge weights.
We assume that each random walk step will cost one unit of the budget\footnote{Our model can be extended to move multiple steps with one unit of budget.}.
Given a total budget constraint $B$ and individual layer budget constraint $c_i$, the MuLaNE task is to find the optimal budget allocation 
$\bk{=}(k_1, ..., k_m)$ with ${\sum_{i=1}^mk_i} \le B$, $0 {\le} k_i {\le} c_i$ such that the
	expected total weights of {\it unique} nodes visited are maximized.
% 	\xutong{relate the model parameters to OSN applications}


In real applications, the network structure $\cG$, the node weights $\bsig$ and the starting distributions $\bm{\alpha}_i$'s may not be known in advance, so we consider both the
	\textit{offline optimization} cases when $\cG$, $\bsig$ and $\bm{\alpha}_i$'s are known and the \textit{online learning} case when $\cG$, $\bsig$ and $\bm{\alpha}_i$'s are unknown.
Moreover, different layers may have overlapping vertices (e.g., home-page of the same user may appear in different OSNs), %(See Figure~\ref{fig: multi-layered}), 
and the starting distributions $\bm{\alpha}_i$'s may or may not be stationary distributions.
In this paper, we provide a systematic study of all these case combinations.

For the offline optimization, we first consider the general overlapping setting and provide constant approximation algorithms based on
	the lattice submodularity property for non-stationary  $\bm{\alpha}_i$'s and the diminishing-return (DR) submodularity property for stationary  $\bm{\alpha}_i$'s.
For the special non-overlapping setting, we design a dynamic programming algorithm that finds the exact optimal solution for MuLaNE.

In the online learning, we conduct multiple rounds of exploration, each of which has the same budget constraints $B$ and $c_i$'s. 
After each round of exploration, the total weights of unique nodes visited in this round are the reward for this round, and
	the trajectory of every explorer in every layer and the importance weights of visited nodes are observed as the feedback, which could be used to learn information about the network for the benefit of future explorations.

We adapt the combinatorial multi-armed bandit (CMAB) framework and the CUCB algorithm \cite{chen2016combinatorial} to our setting, and design online learning algorithms to minimize the regret, which
	is the difference between the cumulative reward achieved by the exact or approximate offline algorithm and that achieved by our learning algorithm,  over $T$ rounds.
We show that directly learning the graph structure $\cG$ is inefficient.
Instead, we define intermediate random variables in MuLaNE as the base arms in CMAB and learn these intermediate parameters, which can sufficiently determine the rewards to guide our budget allocation.
Moreover, the node weight is not revealed until this node is first visited, which further complicates the design of online exploration algorithms.
For the overlapping case, we adapt the CUCB algorithm to address the unrevealed node weights and  the extra constraint of monotonicity for the intermediate parameters.
We further improve the analysis by leveraging on special properties in our setting and show logarithmic regret bounds in this case.
For the non-overlapping case, we define more efficient intermediate parameters and use the exact offline algorithm, and thus achieve a better regret bound. 
% Due to the space limit, all proofs are included in the supplementary material.
%% \vspace{-1pt}
Finally, we conduct experiments on a real-world multi-layered social network dataset to validate the effectiveness of both our offline and online algorithms.

%%\vspace{-1pt}
Our contributions can be summarized as follows: (1) We are the first to model the multi-layered network exploration via random walks problem (\mulane) as an abstraction for many real-world applications (2) We provide a systematic study of the \mulane{} problem via theoretical analysis and empirical validation by considering offline and online settings for both overlapping and non-overlapping multi-layered networks. 
Due to the space limit, proofs are included in the supplementary material.


\input{content/related.tex}


==> MuLaNE Camera Ready ICML2021/content/offline.tex <==
\section{Offline Optimization for \mulane}\label{sec: offline opt}
In this section, we first consider the general case, where layers are overlapping and starting distributions are arbitrary.
Next, we consider the starting distribution is the stationary distribution, and give solutions with better solution quality and time complexity.
Then we analyze special cases where layers are non-overlapping and give optimal solutions for arbitrary distributions.
The summary for offline models and algorithmic results are presented in Table~\ref{tab: offline models}.
\begin{table*}[t]
	\centering
	\caption{Summary of the offline models and algorithms.}	\resizebox{2.05\columnwidth}{!}{
	\label{tab: offline models}
	\begin{tabular}{ccccc}
		\toprule
		\textbf{Overlapping?}& \textbf{Starting distribution}& \textbf{Algorithm} & \textbf{Apprx ratio} & \textbf{Time complexity}\\
		\midrule
		\checkmark & \textit{Arbitrary} & Budget Effective Greedy & %$(1-e^{-\eta})$\footnotemark 
		$(1-e^{-\eta})$\footnote{$1-e^{-\eta}\approx 0.357$, where $\eta$ is the solution of $e^\eta=2-\eta$.}
		&$O(B\norm{\bc}_{\infty}mn_{max}+\norm{\bc}_{\infty}mn_{max}^3)$ \\
		%\checkmark & \textit{Arbitrary} & Budget Effective Greedy & $(1-1/e)$ & $O(B^4\norm{\bc}_{\infty}m^4n_{max} + \norm{\bc}_{\infty}mn_{max}^3)$ \\
		%& & with Partial Enumeration & & \\
		\checkmark & \textit{Stationary} & Myopic Greedy & $(1-1/e)$ & $O(Bmn_{max}+\norm{\bc}_{\infty}mn_{max}^3)$ \\
		$\times$ & \textit{Arbitrary} & Dynamic Programming & 1 & $O(B\norm{\bc}_{\infty}m+\norm{\bc}_{\infty}mn_{max}^3)$ \\
		$\times$ & \textit{Stationary} & Myopic Greedy & 1 & $O(B\log m + \norm{\bc}_{\infty}mn_{max}^3)$ \\
		\bottomrule
	\end{tabular}
}
\end{table*}

\subsection{Overlapping MuLaNE}
\textbf{Starting from arbitrary distributions.}
Based on the equivalent bipartite coverage model, one can observe that our problem formulation is a generalization of the Probabilistic Maximum Coverage (PMC)~\cite{chen2016combinatorial} problem, which is NP-hard and has a $(1-1/e)$ approximation based on submodular set function maximization.
However, our problem is more general in that we want to select multi-sets from $\cW$ with budget constraints, and the reward
	function in general does not have the DR-submodular property for an arbitrary starting distribution.
Nevertheless, we have the following lemma to solve our problem.


\begin{restatable}{lemma}{thmSubmodular}\label{thm: lattice submodular}
For any network $\cG$, distribution $\bm{\alpha}$ and weights $\bsig$, $r_{\cG, \bm{\alpha},\bsig}(\cdot): \bbZ^m_{\ge 0} \rightarrow \R$ is monotone and submodular.
    	%, i.e.,
	%$r_{\cG}(\bm{\alpha}, \bm{x \wedge y}) + r_{\cG}(\bm{\alpha}, \bm{x \vee y}) \le r_{\cG}(\bm{\alpha}, \bm{x}) + r_{\cG}(\bm{\alpha}, \bm{y})$ for any $\bm{x},\bm{y} \in \Z^m_{\ge 0}$, and $r_{\cG}(\bm{\alpha}, \bm{x}) \le r_{\cG}(\bm{\alpha}, \bm{y})$ if $\bm{x} \le \bm{y}$.
\end{restatable}


Leveraging on the monotone submodular property, we design a Budget Effective Greedy algorithm (Alg.~\ref{alg: layer traversal greedy}).
The core of Alg.~\ref{alg: layer traversal greedy} is the BEG procedure.
Let $\delta(i,b, \bk)$ be the \textit{per-unit marginal gain} $(r_{\cG,\bm{\alpha},\bsig}( \bm{k}+b\bm{\chi}_i) - r_{\cG,\bm{\alpha},\bsig}( 
\bm{k}))/b$ for allocating $b$ more budgets to layer $i$, which equals to
\begin{equation}\textstyle\label{eq: marginal gain delta}
 \sum_{u\in \cV}\sigma_u \Pi_{j\neq i}(1-P_{j,u}(k_j))(P_{i,u}(k_i+b)-P_{i,u}(k_i))/b.   
\end{equation}
BEG procedure consists of two parts and maintains a queue $\cQ$, where any pair $(i,b) \in \cQ$ represents a tentative plan of allocating $b$ more budgets to layer $i$.
The first part is built around the while loop (line~\ref{line: alg3 while begin}-\ref{line: remove}), where each iteration greedily selects the $(i,b)$ pair in $\cQ$ such that the \textit{per-unit marginal gain} $\delta(i,b, \bk)$ is maximized.
%If $b$ is less or equal to the remaining budgets, we allocate $b$ more budgets to layer $i$, otherwise we can not extend the current budget allocation and directly enter the next iteration to search the next tentative allocation.
The second part is a for loop (line~\ref{line: alg3 for begin}-\ref{line: alg3 for end}), where in the $i$-th round we attempt to allocate all $c_i$ budgets to layer $i$ and replace the current best budget allocation if we have a larger reward.
\begin{restatable}{theorem}{thmOverSol}\label{thm: overlapping solution}
    Algorithm~\ref{alg: layer traversal greedy} obtains a $(1-e^{-\eta})\approx 0.357$-approximate solution, where $\eta$ is the solution of equation $e^\eta=2-\eta$, to the overlapping MuLaNE problem.
    %with an arbitrary starting distribution.
\end{restatable}
Line 1 uses $O(m\norm{\bc}_{\infty}n_{max}^3)$ time to pre-calculate visiting probabilities based on Eq.~(\ref{eq: simple form}), 
where $n_{max}=\max_{i}|\cV_i|$.
In the BEG procedure, the while loop contains $B$ iterations, the size of queue $\cQ$ is $O(m\norm{\bc}_{\infty})$, and line~\ref{line: largest margin} uses $O(n_{max})$ to calculate $\delta(i,b,\bk)$ by proper pre-computation and update\OnlyInFull{ (see Appendix~\ref{appendix: efficient eval})}, 
thus the time complexity of Algorithm~\ref{alg: layer traversal greedy} is $O(B\norm{\bc}_{\infty}mn_{max} + m\norm{\bc}_{\infty}n_{max}^3)$.

\noindent\textbf{Remark 1.} The idea of combining the greedy algorithm with enumerating solutions on one layer is also adopted in previous works~\cite{khuller1999budgeted, alon2012optimizing}, but
they only give a $\frac{1}{2}(1-e^{-1}) \approx 0.316$-approximation analysis. 
In this paper, we provide a novel analysis with a better $(1-e^{-\eta})\approx 0.357$-approximation, \OnlyInFull{see Appendix~\ref{appendix: offline proof arbitrary distribution} for details}.

\noindent\textbf{Remark 2.} Another algorithm~\cite{alon2012optimizing} with a better approximation ratio is to use partial enumeration techniques (i.e., BEGE), which can achieve $(1-1/e)$ approximation ratio.
This is the best possible solution in polynomial time unless P=NP.
But the time complexity is prohibitively high in $O(B^4m^4\norm{\bc}_{\infty}n_{max}+ m\norm{\bc}_{\infty}n_{max}^3)$.
\OnlyInFull{The algorithm and the analysis are provided in the Appendix~\ref{appendix: enum begreedy analysis}.}



\begin{algorithm}[t]
	\caption{Budget Effective Greedy (BEG) Algorithm for the Overlapping MuLaNE}\label{alg: layer traversal greedy}
	\resizebox{.97\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \INPUT Network $\cG$, starting distributions $\bm{\alpha}$, node weights $\bsig$, budget $B$, constraints $\bc$.
	    \OUTPUT Budget allocation $\bk$.
	    \STATE Compute visiting probabilities $(P_{i,u}(b))_{i\in[m], u\in\cV, b \in [c_i]}$ according to Eq.~(\ref{eq: simple form}). \label{line:computePiub}
	    \STATE $\bk \leftarrow$ BEG($(P_{i,u}(b))_{i\in[m], u\in\cV, b \in [c_i]}$,$\bsig$, $B$, $\bc$). \label{line:return}
	    \algrule
		\FUNCTION {BEG($(P_{i,u}(b))_{i\in[m], u\in\cV, b \in [c_i]}$, $\bsig$, $B$, $\bc$)}
		\STATE Let $\bm{k}\defeq(k_1, ..., k_m) \leftarrow \bm{0}$, $K\leftarrow B$. \label{line:test} 
		\STATE Let $\cQ \leftarrow \{(i,b_i) \, | \, i \in [m], 1\le b_i \le  c_i\}$.
		\WHILE {$K > 0$ and $\cQ \neq \emptyset$ \label{line: alg3 while begin}}
		    \STATE $(i^*,b^*) \leftarrow \argmax_{(i,b)\in \cQ} \delta(i,b,\bk)/b$ \label{line: largest margin} \algorithmiccomment{Eq.~(\ref{eq: marginal gain delta})}
		    \STATE $k_{i^*} \leftarrow k_{i^*} + b^*$, $K \leftarrow K - b^*$.
		    \STATE Modify all pairs $(i,b) \in \cQ$ to $(i, b - b^*)$.
		    \STATE Remove all paris $(i,b) \in \cQ$ such that $b \le 0$.\label{line: remove}
		\ENDWHILE
		%\State $\bm{k^*} = \argmax_{i\in[m]}r_{\cG}(\bm{\alpha}, B\bm{\chi}_i)$
		\FOR{$i \in [m]$} \label{line: alg3 for begin}
		\STATE \textbf{if} $r_{\cG,\bm{\alpha},\bsig}( c_i\bm{\chi}_i) > r_{\cG,\bm{\alpha},\bsig}( \bm{k})$, \textbf{then} $\bk \leftarrow c_i \bch_i.$ \label{line: alg3 for end}
		\ENDFOR
		\STATE \textbf{return} $\bk\defeq(k_1, ..., k_m)$.
		\ENDFUNCTION
		\end{algorithmic}
		\end{minipage}}
\end{algorithm}

\noindent\textbf{{Starting from the stationary distribution.}}
We also consider the special case where each random explorer $W_i$ starts from the stationary distribution $\bm{\pi_i}$
	with $\bm{\pi_i}^{\top} \bP = \bm{\pi_i}^{\top}$.
%If a Markov chain $\bP$ admits a stationary distribution $\bm{\pi}$, the random walk will gradually approach $\bm{\pi}$ from arbitrary starting distributions.
%Furthermore, in the random walk literature, the stationary distribution often gives nice properties for the theoretical analysis.
In this case, we have the following stronger DR-submodularity.

\begin{restatable}{lemma}{thmDRSubmodular}
	For any network $\cG$, stationary distributions $\bm{\pi}$ and node weights $\bsig$, function $r_{\cG,\bm{\pi},\bsig,}(\cdot):\bbZ^m_{\ge 0} \rightarrow \R$ is monotone and DR-submodular.
	%, i.e.,
	%$r_{\cG}(\bm{\pi}, \bm{y} + \bm{\chi_j}) - r_{\cG}(\bm{\pi}, \bm{y}) \le r_{\cG}(\bm{\pi}, \bm{x}+\bm{\chi_j)} - r_{\cG}(\bm{\pi}, \bm{x})$, and $r_{\cG}(\bm{\pi}, \bm{x}) \le r_{\cG}(\bm{\pi}, \bm{y})$ for any $\bm{x} \le \bm{y}$, $j\in [m]$.
\end{restatable}
Since the reward function is DR-submodular, 
the BEG procedure can be replaced by 
the simple MG procedure in Alg.~\ref{alg: pure greedy} with a better approximation ratio.
The time complexity is also improved to $O(Bmn_{max}+m\norm{\bc}_{\infty}n_{max}^3)$.
% \footnotetext{$1-e^{-\eta}\approx 0.357$, where $\eta$ is the solution of $e^\eta=2-\eta$.}
% \OnlyInFull{\vspace{-10pt}}
%First, line~\ref{eq: largest margin} always select the pair $(i^*, b^*)$ such that $b^*=1$ because %$r_{\cG}(\bm{\alpha}, \bm{k}+b\bm{\chi}_i) - r_{\cG}(\bm{\alpha}, \bm{k}+(b-1)\bm{\chi}_i) \le r_{\cG}(\bm{\alpha}, \bm{k}+\bm{\chi}_i) - r_{\cG}(\bm{\alpha}, \bm{k})$ for arbitrary $\bk$, $i$ and $b$.
%$\delta(i,b+1,\bk) \le \delta(i,b, \bk)$
%for arbitrary $\bk$, $i$ and $b\ge 1$.
%Thus, Alg.~\ref{alg: layer traversal greedy} can always  
%extend the current budget allocation $\bk$ by $1$ and never enters line~\ref{line: remove}.
%Therefore, line~\ref{line: remove} and lines~\ref{line: alg3 for begin}-\ref{line: alg3 for end} can be safely removed.
%Following the similar argument to the proof of Thm.~\ref{thm: overlapping solution}, we can show that the following theorem holds.
\begin{restatable}{theorem}{thmOverStationarySol}
    Algorithm ~\ref{alg: pure greedy} obtains a $(1-1/e)$-approximate solution to the overlapping
    MulaNE with the stationary starting distributions.
\end{restatable}
% \OnlyInFull{\vspace{-10pt}}
%
%because Alg~\ref{alg: pure greedy} runs for $B$ iterations and each iteration requires $O(m\theta_2)$ to locate the layer $i$ with the largest one step marginal gain $\delta(i,1,\bk)$. %$\left(r_{\cG}(\bm{\alpha}, \bm{k}+\bm{\chi}_i) - r_{\cG}(\bm{\alpha}, \bm{k})\right)$.



\begin{algorithm}[t]
\caption{Myopic Greedy (MG) Algorithm for MuLaNE }\label{alg: pure greedy}
\resizebox{.95\columnwidth}{!}{
\begin{minipage}{\columnwidth}
\begin{algorithmic}[1]
\STATE Same input, output and line~\ref{line:computePiub}-\ref{line:return} as in Alg.~\ref{alg: layer traversal greedy}, except replacing BEG with MG procedure below.
\algrule
\FUNCTION{MG($(P_{i,u}(b))_{i\in[m], u\in\cV, b \in [c_i]}$, $\bsig$, $B$, $\bc$)}
\STATE Let $\bm{k}\defeq(k_1, ..., k_m) \leftarrow \bm{0}$, $K \leftarrow B$.\;
\WHILE{$K  > 0$} 
    \STATE $i^*\leftarrow\argmax_{i \in [m], k_i + 1 \le c_i} \delta(i,1,\bk).$  \algorithmiccomment{Eq.~(\ref{eq: marginal gain delta})}
    %\tcc{$O(\log m)$ using the priority queue}
    \label{line: greedy select}
    \STATE $k_{i^*} \leftarrow k_{i^*} + 1$, $K \leftarrow K - 1$.\;
    \ENDWHILE
    \STATE \textbf{return} {$\bk=(k_1, ..., k_m)$.}
\ENDFUNCTION
\end{algorithmic}
\end{minipage}}
\end{algorithm}

% \vspace{-10pt}
\subsection{Non-overlapping MuLaNE}
For non-overlapping MuLaNE, we are able to achieve the exact optimal solution: for the stationary starting distribution, a slight modification of the greedy algorithm Alg.~\ref{alg: pure greedy} gives the optimal solution, while for an arbitrary starting distribution,
we design a dynamic programming algorithm to compute the optimal solution \OnlyInShort{(see supplementary material)}.
\OnlyInFull{Due to the space constraint, the details are included in Appendix~\ref{appendix: offline non over analysis}.}

%
%we still consider two different starting distributions and give \textit{optimal}, rather than approximate solutions, based on Dynamic Programming (Alg.~\ref{alg: dynamic programming}) and Greedy (Alg.~\ref{alg: pure greedy}) Algorithms, respectively.
%Due to the space limitation, we provide the algorithms, analysis and proofs in the Appendix~\ref{appendix: offline non over analysis}.


==> MuLaNE Camera Ready ICML2021/content/online.tex <==
%%\OnlyInFull{\vspace{-5pt}}
\section{Online Learning for \mulane}\label{sec: online learning}
%%\OnlyInFull{\vspace{-5pt}}
In the online setting, we continue to study both overlapping and non-overlapping \mulane{} problem.
However, the network structure $\cG$, the distribution $\bm{\alpha}$ and node weights $\bsig$ \textit{are not known a priori}. 
Instead, the only information revealed to the decision maker includes total budget $B$, the number of layers $m$, the number of the target nodes $|\cV|$ (or an upper bound of it) and the budget constraint $\bc$.
% \xutong{
% As to be explained below, for unknown network structure, our solution would be estimating certain intermediate parameters, instead of estimating the graph structure (namely
% 	the transition probability matrix $\bm{P}_i$) and the starting distribution $\bm{\alpha}$.
% For unknown node weight $\sigma_u$, we maintain an optimistic weight before we first visit $u$. 
% }
% With a little abuse of the notation, we use $\bm{\mu}$ to denote the unknown intermediate parameters and $r_{\bm{\mu}, \bsig}(\bk)$ to denote the reward $r_{\cG, \bm{\alpha}, \bsig}(\bk)$.


\subsection{Online Algorithm for Overlapping \mulane}
% To deal with the unknown network structure, one possible method is to estimate the transition probability matrix $\bm{P}_i$ for each layer. 
% But this approach has two issues:
% First, it is hard to analyze how the estimated $\bm{\hat{P}}_i$ affects the performance of online algorithms since we consider general graph structures whose reward function given by Eq.~(\ref{eq: over reward}) is highly non-linear.
% Second, extensive matrix calculation are needed in each round, which can be inefficient for large networks.

For the unknown network structure and starting distributions, we bypass the transition matrices $\bm{P}_i$ and directly estimate the visiting probabilities $P_{i,u}(b) \in [0,1]$.
This avoids the analysis for how the estimated $\bm{{P}}_i$ affects the performance of online algorithms, which could be unbounded since we consider general graph structures and the reward function given by Eq.~(\ref{eq: over reward}) is highly non-linear in $\bm{{P}}_i$.
Moreover, we can save the matrix calculation by directly using $P_{i,u}(b)$, which is efficient even for large networks.

Specifically, we maintain a set of base arms $\cA = \{(i,u,b)| i \in [m], u \in \cV, b \in [c_i]\}$, where the total number $|\cA| = \sum_{i \in [m]}c_i|\cV|$.
For each base arm $(i,u,b) \in \cA$, we denote $\mu_{i,u,b}$ as the true value of each base arm, i.e., 
$\mu_{i,u,b}=P_{i,u}(b)$.
For the unknown node weights, we maintain the optimistic weight $\bar{\sigma}_u=1$ if $u \in \cV$ has not been visited.
After $u$ is first visited and its true value $\sigma_u$ is revealed, we replace $\bar{\sigma}_u$ with $\sigma_u$.
With a little abuse of the notation, we use $\bm{\mu}$ to denote the unknown intermediate parameters and $r_{\bm{\mu}, \bsig}(\bk)$ to denote the reward $r_{\cG, \bm{\alpha}, \bsig}(\bk)$.

We present our algorithm in Alg.~\ref{alg: over online}, which is an adaptation of the CUCB algorithm for the general
	Combinatorial Multi-arm Bandit (CMAB) framework~\cite{chen2016combinatorial} to our setting.
Notice that we use $\cA$ as defined above in the algorithm, and $\cA$ is defined using $\cV$, which is the set of node ids and 
	should not be known before the learning process starts.
This is not an issue, because at the beginning we can create $|\cV|$ (which is known) placeholders for the node ids, and once a new node is visited,we 
	immediately replace one of the placeholders with the new node id.
Thus $\cV$ appearing in the above definition of $\cA$ is just for notational convenience.


In Alg.~\ref{alg: over online}, we maintain an unbiased estimation of the visiting probability $P_{i,u}(b)$, denoted as $\hat{\mu}_{i,u,b}$.
Let $T_{i,u,b}$ record the number of times arm $(i,u,b)$ is played so far and $\bar{\sigma}_v$ denote the optimistic importance weight.
In each round $t \ge 1$, we compute the confidence radius $\rho_{i,u,b}$ in line~\ref{line: over online radius}, which controls the level of exploration.
%, where $\gamma \ge 0$ is the exploration parameter controlling the level of exploration.
The confidence radius is larger when the arm $(i,u,b)$ is not explored often (i.e. $T_{i,u,b}$ is small), and thus motivates more exploration. 
%In line~\ref{line: over online ucb}, we compute the upper confidence bound (UCB) value $\tilde{\mu}_{i,u,b}$. 
Due to the randomness of the exploration process, the upper condifence bound (UCB) value $\tilde{\mu}_{i,u,b}$ could be decreasing w.r.t $b$, but our offline oracle BEG can only accept non-decreasing UCB values (otherwise the $1-e^{-\eta}$ approximation is not guaranteed).
Therefore, in line~\ref{line: over online validate}, we increase the UCB value $\tilde{\mu}_{i,u,b}$ and set it to be $\max_{j \in [b]} {\tilde{\mu}_{i,u,j}}$. 
This is the adaption of the CUCB algorithm to fix our case, and thus we name our algorithm as CUCB-MAX.
%\{The following example could be removed if we need space.}
%Consider two base arms $a_1 = (i,u,b_1)$ and $a_2 = (i,u,b_2)$, $b_1 < b_2$, 
%arm $a_2$ has both larger true value and larger confidence radius ($T_{i,u,b_2}$ is smaller due to line~\ref{line: over online update}), so it is safe to increase $a_2$'s UCB value if it is smaller than $a_1$'s.
After we apply the $1-e^{-\eta}$ approximate solution $\bk$ given by the BEG oracle (i.e., Alg.~\ref{alg: layer traversal greedy}), we get $m$ trajectories as feedbacks.
In line~\ref{line: update weight}, we can update the unknown weights of visited nodes. In line~\ref{line: over online update}, for base arms $(i,u,b)$ with $b \le k_i$, we update corresponding statistics by the Bernoulli random variable $Y_{i,u,b}\in\{0,1\}$ indicating whether node $u$ is visited by $W_i$ in first $b$ steps.

\begin{algorithm}[t]
	\caption{CUCB-MAX Algorithm for the \mulane}\label{alg: over online}
	\resizebox{.97\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \INPUT{Budget $B$, number of layers $m$, number of nodes $|\cV|$, constraints $\bc$, offline oracle BEG.}
		\STATE For each arm $(i,u,b) \in \cA$, $T_{i,u,b} \leftarrow 0$, $\hat{\mu}_{i,u,b} \leftarrow 0$. %\tcc{maintain the total number of times arm $(i,u,b)$ is played so far}
		%For each arm $(i,u,b)$, $\hat{\mu}_{i,u,b} \leftarrow 1$ \;
		%\tcc{maintain the empirical mean of marginal gain $P_{i,u}(b)$}
		\STATE {For each node $v \in \cV$, $\bar{\sigma}_v \leftarrow 1$.}
		\FOR {$t=1,2,3,...,T $}
		    \FOR {$(i,u,b) \in \cA$}
		    \STATE $\rho_{i,u,b} \leftarrow \sqrt{3\ln t/(2T_{i,u,b})}$.  \label{line: over online radius}
		    %\tcc{the confidence radius, $\rho_{i,b} \leftarrow +\infty$, when $T_{i,u,b} = 0.$}
		    \STATE $\tilde{\mu}_{i,u,b} \leftarrow \min \{\hat{\mu}_{i,u,b} + \rho_{i,u,b}, 1\}$. 
		    %\tcc{the upper confidence bound}
		    \label{line: over online ucb}
            \ENDFOR
        \STATE For $(i,u,b)\in \cA$, $\bar{\mu}_{i,u,b} \leftarrow \max_{j \in [b]} {\tilde{\mu}_{i,u,j}}$.		%\tcc{guarantee the ucb value is monotone} 
		\label{line: over online validate}\label{alg: valid}
		\STATE $\bm{k} \leftarrow$ BEG($(\bar{\mu}_{i,u,b})_{(i,u,b)\in\cA}$, $(\bar{\sigma}_v)_{v \in \cV}$, $B$, $\bc$).
		%\tcc{Budget allocation $\bm{k}$, exploration trajectories $\bm{X}$}
		\label{line: over online oracle}
		\STATE Apply budget allocation $\bk$, which gives trajectories $\bm{X}\defeq(X_{i,1}, ..., X_{i,k_i})_{i\in [m]}$ as feedbacks. \label{line: over online feedback}
		\STATE { For any visited node $v \in \bigcup_{i\in[m]}\{X_{i,1}, ..., X_{i,k_{i}}\}$, receive its node weight $\sigma_v$ and set $\bar{\sigma}_v \leftarrow \sigma_v$. }\label{line: update weight}
		\STATE For any $(i,u,b) \in \tau \defeq \{(i,u,b) \in \cA \vert \, b \le k_i\}$, \\$Y_{i,u,b} \leftarrow 1$ if $u \in \{X_{i,1}, ..., X_{i, b}\}$ and $0$ otherwise.\label{line: over bernoulli rv}
		\STATE For $(i,u,b) \in \tau$, update $T_{i,u,b}$ and $\hat{\mu}_{i,u,b}$:\\ 
		$T_{i,u,b} \leftarrow T_{i,u,b} + 1$,  $\hat{\mu}_{i,u,b} \leftarrow \hat{\mu}_{i,u,b} + (Y_{i,u,b} - \hat{\mu}_{i,u,b})/T_{i,u,b}.$\label{line: over online update}
		\ENDFOR
		\end{algorithmic}
    		\end{minipage}}
\end{algorithm}



\noindent\textbf{{Regret Analysis.}}
We define the reward gap $\Delta_{\bm{k}}{=}\max(0, \xi r_{\bm{\mu}, \bsig}(\bm{k^*}) - r_{\bm{\mu}, \bsig}(\bm{k}))$ for all feasible action $\bm{k}$ satisfying $\sum_{i=1}^{m}k_i = B$, $0 \le k_i \le c_i$, where $\bk^*$ is the optimal solution for parameters $\bm{\mu}$, $\bsig$ and
	$\xi=1-e^{-\eta}$ is the approximation ratio of the $(\xi,1)$-approximate offline oracle. For each base arm $(i,u,b)$, 
we define  $\Delta_{\min}^{i,u,b}{=}\min_{\Delta_{\bm{k}}>0, k_i = b}\Delta_{\bm{k}}$ and $\Delta_{\max}^{i,u,b}{=}\max_{\Delta_{\bm{k}}>0, k_i=b}\Delta_{\bm{k}}$. 
As a convention, if there is no action $\bm{k}$ with $k_i=b$ such that $\Delta_{\bm{k}} {>} 0$, we define $\Delta_{\min}^{i,u,b}{=}\infty$ and $\Delta_{\max}^{i,u,b}{=}0$. 
Let $\Delta_{\min} {=} \min_{(i,u,b) \in \cA}\Delta_{\min}^{i,u,b}$ and $\Delta_{\max} {=} \max_{(i,u,b) \in \cA}\Delta_{\max}^{i,u,b}$.
The following theorem summarizes the regret bound for Alg.~\ref{alg: over online}.
\vspace{-0pt}
\begin{restatable}{theorem}{thmOver} \label{thm: over regret}
%When $\gamma \ge 1$, 
Algorithm~\ref{alg: over online} has the following distribution-dependent $(1-e^{-\eta}, 1)$ approximation regret,
\begin{equation*}\textstyle
Reg_{\bm{\mu}, \bsig}(T) \le \sum_{(i,u,b) \in \cA}\frac{108m|\cV| \ln T}{\Delta_{\min}^{i,u,b}} + 2|\cA| + \frac{\pi^2}{3}|\cA|\Delta_{\max}.
\end{equation*}
%and the distribution-independent $(1-e^{-\eta}, 1)$ approximation regret bound,
%\begin{equation*}\textstyle
%	Reg_{\bm{\mu}}(T) \le  14\sqrt{\gamma^2m|\cV||\cA|T\ln T} + 2|\cA|+ \frac{\pi^2}{3}|\cA|\Delta_{\max}.
%\end{equation*}
\end{restatable}
% \vspace{-5pt}
\noindent\textbf{Remark 1.}
Looking at the above distribution dependent bound, we have the $O(\log T)$ approximation regret, which is asymptotically tight.
% Parameter $\gamma$ is the exploration parameter used later to tune our experiments, and $\gamma=1$ is the smallest value to have the above theoretical guarantee.
Coefficient $m|\cV|$ in the leading term corresponds to the number of edges in the complete bipartite coverage graph. Notice that we cannot use the true edge number $\sum_{i \in [m]}{|\cV_i|}$, 
	because the learning algorithm does not know which nodes are contained in each layer, and has to explore all visiting
	possibilities given by the default complete bipartite graph.
The set of base arms $\cA$ has some redundancy due to the correlation between these base arms, and thus it is unclear 
	if the summation over all base arms in the regret bound is tight.
For the non-overlapping case, we further reduce the number of base arms to achieve better regret bounds, but for the overlapping case,
	how to further reduce base arms to achieve a tighter regret bound is a challenging open question left for the future work.

\noindent\textbf{Remark 2.}
The $(1-e^{-\eta}, 1)$ approximate regret is determined by the offline oracle BEG that we plug in Line~\ref{line: over online oracle} and can be replaced by $(1-1/e, 1)$ regret using BEGE or even by the exact regret if the oracle can obtain the optimal budget allocation.
The usage of BEG is a trade-off we make between computational efficiency and learning efficiency and empirically, it performs well as we shall see in Section~\ref{sec: experiments}. 

\noindent\textbf{Remark 3.} %The proofs of the above theorem is an adaption of the proof of Theorem 4 in~\cite{wang2017improving}, and the full proofs are included in the \OnlyInFull{Appendix~\ref{appendix: over online analysis}}\OnlyInShort{Appendix E}.
The full proof of the above theorem is included in the
\OnlyInFull{Appendix~\ref{appendix: over online analysis}}\OnlyInShort{supplementary material}, where we rely on the following properties of $r_{\bm{\mu}, \bsig}(\bk)$ to bound the regret.

%omit
\begin{restatable}{property}{condOverMono}(Monotonicity). \label{cond: over mono}
	The reward $r_{\bm{\mu}, \bsig}(\bm{k})$ is monotonically increasing, i.e., 
	for any budget allocation $\bm{k}$, any two vectors $\bm{\mu} {=} (\mu_{i,u,b})_{(i,u,b)\in \cA}$, $\bm{\mu'}{=}(\mu'_{i,u,b})_{(i,u,b) \in \cA}$ and any node weights $\bsig$, $\bsig'$, we have $r_{\bm{\mu}, \bsig}(\bm{k}) \le r_{\bm{\mu'}, \bsig'}(\bm{k})$, if $\mu_{i,u,b} \le \mu'_{i,u,b}$ and $\sigma_v \le \sigma'_v$, $\forall (i,u,b) \in \cA, v \in \cV$.
\end{restatable}
\begin{restatable}{property}{condOverOneNorm}(1-Norm Bounded Smoothness).\label{cond: over 1-norm}
	The reward function $r_{\bm{\mu}, \bsig}(\bm{k})$ satisfies the 1-norm bounded smoothness condition, i.e., 
	for any budget allocation $\bm{k}$, any two vectors $\bm{\mu} {=} (\mu_{i,u,b})_{(i,u,b)\in \cA}$, $\bm{\mu'}{=}(\mu'_{i,u,b})_{(i,u,b) \in \cA}$ and any node weights $\bsig$, $\bsig'$, we have $|r_{\bm{\mu}, \bsig}(\bm{k}) - r_{\bm{\mu'}, \bsig'}(\bm{k})| \le \sum_{i \in [m], u \in \cV, b = k_i}(\sigma_u|\mu_{i,u,b} - \mu'_{i,u, b}|+\abs{\sigma_u-\sigma_u'}\mu'_{i,u,b})$.
\end{restatable}
We emphasize that our algorithm and analysis differ from the original CUCB algorithm~\cite{, chen2016combinatorial} as follows.
First,  we have the additional regret caused by the over-estimated weights for unvisited nodes, i.e., $\abs{\sigma_u-\sigma_u'}\mu'_{i,u,b}$ term in~ property \ref{cond: over 1-norm}.
We carefully bound this term based on the observation that $\mu'_{i,u,b}$ is small and decreasing quickly before $u$ is first visited.
Next, we have to take the max (line~\ref{line: over online validate}) to guarantee the UCB value is monotone w.r.t $b$ since our BEG oracle can only output $(1-e^{-\eta},1)$-approximation with monotone inputs. 
Due to the above operation, $(i,u,b)$'s UCB value depends on the feedback from all arms $(i,u,j)$ for $j \le b$
	(set $\tau$ in line~\ref{line: over bernoulli rv}).
% 	\wei{It is strange that when I click the line number above, it does not go to line 9 of Algo 3, but line 9 of Algo 1? I do not know the reason, but it is better to fix this, otherwise, a reviewer may get confused if he clicks the link.}
	 So we should update 
	all these arms (line~\ref{line: over online update}) to guarantee that the estimates to all these arms are accurate enough.
Finally, directly following the standard CMAB result would have a larger regret, because arms in $\tau$ are defined as triggered arms, but only arms in $\tau'=\{(i,u,b)\in \cA| k_i=b\}$ affect the rewards.
So we conceptually view arms in $\tau'$
% 	\wei{``these'' means arms in $\tau'$ or $\tau$?}
 as triggered arms and use a tighter 1-Norm Bounded Smoothness condition as given above 
	to derive a tighter regret bound.
This improves the coefficient of the leading $\ln T$ term in the distribution dependent regret by a factor of $|\tau|/|\tau'|= O(B/m)$, and the $1/\Delta_{\min}^{i,u,b}$ term is smaller since the original definition would have $\Delta_{\min}^{i,u,b}=\min_{\Delta_{\bm{k}}>0, b \le k_i}\Delta_{\bm{k}}$.

%%\vspace{-3pt}
\subsection{Online Algorithm for Non-overlapping Case} \label{sec:cucbmg}
%%\vspace{-2pt}
For the non-overlapping case, we set \textit{layer-wise marginal gains} as our base arms.
Concretely, we maintain a set of base arms $\cA = \{(i,b) | i \in [m], b \in [c_i]\}$.
For each base arm $(i,b) \in \cA$., let $\mu_{i,b}=\sum_{u \in \cV}\sigma_u(P_{i,u}(b)-P_{i,u}(b-1))$
	be the true marginal gain of assigning budget $b$ in layer $i$.
We apply the standard CUCB algorithm to this setting 
	and call the resulting algorithm CUCB-MG \OnlyInFull{(Algorithm~\ref{alg: non-over online} in Appendix~\ref{appendix: non over online})}\OnlyInShort{(see supplementary material)}.
Note that in the non-overlapping setting we can solve the offline problem exactly, so we can use the exact offline oracle to
	solve the online problem and achieve an exact regret bound.
This is the major advantage over the overlapping setting where we can only achieve an approximate bound.
Define $\Delta_{\bm{k}}=r_{\bm{\mu}, \bsig}(\bm{k^*}) - r_{\bm{\mu}, \bsig}(\bm{k})$ for all feasible action $\bm{k}$,
and $\Delta_{\min}^{i,b}=\min_{\Delta_{\bm{k}}>0, k_i \ge b}\Delta_{\bm{k}}$, 
% \wei{Why the subscript is $k_i \ge b$, just want to confirm.}
CUCB-MG has a $O(\sum_{(i,b) \in \cA}{48B \ln T}/{\Delta_{\min}^{i,b}})$ regret bound.
% \begin{restatable}{theorem}{thmNonOVer} \label{thm: non over regret bound}
% 	When $\gamma \ge 1$, 
% %	\OnlyInFull{Algorithm~\ref{alg: non-over online}}\OnlyInShort{Algorithm 8} 
% 	CUCB-MG
% 	has the following distribution-dependent regret bound,
% 	\begin{equation*}\textstyle
% 	Reg_{\mu}(T) \le \sum_{(i,b) \in \cA}\frac{48\gamma^2 B \ln T}{\Delta_{\min}^{i,b}} + 2|\cA| + \frac{\pi^2}{3}|\cA|\Delta_{\max}.
% 	\end{equation*}
% 	%and the following distribution-independent regret bound,
% 	%\begin{equation*}\textstyle
% 	%Reg_{\mu}(T) \le  14\sqrt{\gamma^2 B|\cA|T\ln T} + 2|\cA| + \frac{\pi^2}{3}|\cA|\Delta_{\max}.
% 	%\end{equation*}
% %	where $\Delta_{\textbf{k}}=r_{\textbf{k}*}(\mu)-r_{\textbf{k}}(\mu)$ for all action $\bm{k}$, $\Delta_{\min}^{i,b}=\min_{\Delta{\textbf{k}}>0, k[i] \ge b}\Delta_{\textbf{k}}$, $\Delta_{\max}^{i,b}=\max_{\Delta{\textbf{k}}>0, k[i]\ge b}\Delta_{\textbf{k}}$, $\Delta_{\max}=\max_{i\in m, b \in B}\Delta_{\max}^{i,b}$
% \end{restatable}  

% \textbf{Remark.} We can compare the regret bound given by Alg.~\ref{alg: over online} and Alg.~\ref{alg: non-over online} when $\gamma = 1$.  
% The distribution-independent bound of Alg.~\ref{alg: non-over online} is $O\left(\sqrt{Bm\norm{\bc}_{\infty}T\ln T}\right)$.
% while the distribution-independent bound of Alg.~\ref{alg: over online} is $O\left(\sqrt{\norm{\bc}_{\infty}(m|\cV|)^2T\ln T}\right)$.
% When $|\cV|>\sqrt{B/m}$, Alg~\ref{alg: non-over online} is favorable  because it has smaller regret.
% This means Alg~\ref{alg: non-over online} is better when the size of non-overlapping multi-layered network $\cG$ is large, due to the fact that the number of base arms for $|\cA|$ decreases from $\sum_{i\in[m]}c_i|\cV|$ to $\sum_{i\in [m]}c_i$, compared to Alg.~\ref{alg: over online}.
% \textbf{Remark 3.} Under stationary starting distribution condition and two other conditions (todo), we can derive the constant distribution-dependent regret bounds by reusing the historical information.
% \begin{restatable}{theorem}{thmConstant}\label{thm: constant}
% 	For the full feedback setting with above revision, Algo.~\ref{CombUCB-CERW} gives the following constant regret bound, 
% 	\begin{equation}\textstyle
% 	Reg_{\bm{\mu}}(T) \le \left[m+2B\sum_{i\in [m]}c_i + \sum_{(i,b) \in [m]\times[B]} \frac{576c_iB^2m^2(\tau_i(\epsilon)+b)}{\Delta_{\min}^2}\right]\Delta_{\max}.
% 	\end{equation}
% 	where $\tau_i(\epsilon)$ is the $\epsilon$-mixing time for $\bm{P}_i$ and $c_i$ is a constant (See Fact~\ref{fact: dependent bound} in Appendix~\ref{app: fact2}).
% \end{restatable}



==> MuLaNE Camera Ready ICML2021/content/preliminary.tex <==
%% \vspace{-5pt}
\section{Problem Settings}\label{sec: problem setting}

\textbf{Basic Notations}.
In this paper, we use $\R$ and $\Z$ to denote the sets of real numbers and integers, respectively, and
	the associated subscript $\ge 0$ and $>0$ denote their non-negative and positive subsets, respectively.
Suppose we want to explore a multi-layered network $\cG(\cV, \cE, \bsig)$, consisting of $m$ layers $L_1, ..., L_m$ and $N$ unique nodes $\cV$ with fixed node weights
$\bsig\in [0,1]^{\cV}$.
Let $[m]$ denote the set $\{1,2,...,m\}$.
Each layer $L_i, i \in[m]$, represents a subgraph of $\cG$ we could explore and is modeled as a weighted digraph $\cG_i(\cV_i, \cE_i;w_i)$,
where $\cV_i \subseteq \cV$ is the set of vertices in layer $L_i$, $\cE_i \subseteq \cV_i\times \cV_i$ is the set of edges in $\cG_i$, 
and $w_i: \cE_i \rightarrow \R_{> 0}$ is the edge weight function associating each edge of $\cG_i$.
For any two layers $L_i$ and $L_j$, we say they are \textit{non-overlapping} if  $\cV_i \cap \cV_j = \emptyset$. 
$\cG$ is called a \textit{non-overlapping} multi-layered network if any two layers are non-overlapping; 
otherwise $\cG$ is an \textit{overlapping} multi-layered network. 
%Figure~\ref{fig: multi-layered} illustrates these two types of networks. 
Let $n_i=|\cV_i|$ denote the size of layer $L_i$, and 
the adjacency matrix of $\cG_i$ is defined as $\bm{A_i} \in \R^{n_i \times n_i}_{\ge 0}$, where
$\bm{A_i}[u,v]=w_i((u,v))$ if $(u,v)\in \cE_i$ and 0 otherwise. 
% Based on the definition of $\bm{A_i}$, we also define the transition probability matrix	$\bm{P}_i \in \R^{n_i \times n_i}_{\ge 0}$ as $\bm{P}_i{[u,v]} \defeq \bm{A_i}{[u,v]}/(\sum_{w:{(u,w)} \in \cE_i} \bm{A_i}{[u,w]} )$.

%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/multi-layer/multi-layer_bold.eps}
%         \caption{Overlapping.}
%         \label{fig: over}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.23\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/multi-layer/non_over_multi_layered.eps}
%         \caption{Non-overlapping.}
%         \label{fig: non-over}
%     \end{subfigure}
%        \caption{Two types of multi-layered networks.}
%        \label{fig: multi-layered}
%\end{figure}
\noindent\textbf{Exploration Rule.}
Each layer $L_i$ is associated with an explorer $W_i$, a budget $k_i \in \Z_{\ge 0}$ and an initial starting distribution 
$\bm{\alpha}_i = (\alpha_{i,u})_{u\in \cV_i}\in \R^{n_i}_{\ge 0}$ with $\sum_{u\in \cV_i} \alpha_{i,u}=1$.
The exploration process of $W_i$ is identical to applying \textit{weighted random walks} within layer $L_i$. 
Specifically, the explorer $W_i$ starts the exploration from a random node $v_1\in \cV_i$ with probability $\alpha_{i,v_1}$; 
it consumes one unit of budget and continues the exploration by walking
from $v_1$ to one of its out-neighbors, say $v_2$, with probability $\bm{P}_i[v_1, v_2]$, where $\bm{P}_i \in \R^{n_i \times n_i}_{\ge 0}$ is the transition probability matrix, and $\bm{P}_i{[u,v]} {\defeq} \bm{A_i}{[u,v]}/(\sum_{w:{(u,w)} \in \cE_i} \bm{A_i}{[u,w]} )$. 
Consider visiting the initial node $v_1$ as the first step, the process is repeated until the explorer $W_i$ walks $k_i$ steps
 and visits $k_i$ nodes (with possibly duplicated nodes).
Note that one can easily generalize our results by moving $\lambda_i \in \bbZ_{>0}$ steps with one unit of budget for $W_i$, 
%One can easily verify that this modification will not affect our algorithm and the analysis, 
and for simplicity, we set $\lambda_i=1$.

\noindent\textbf{Reward Function.}
We define the exploration trajectory for explorer $W_i$ after exploring $k_i$ nodes as $\Phi(i,k_i) {\defeq}(X_{i,1}$, $\ldots, X_{i,k_i})$, where $X_{i,j} \in \cV_i$ denotes the node visited at $j$-th step, and $\Pr(X_{i, 1}{=}u) = \alpha_{i,u}, u\in \cV_i$.
%Note that $\alpha_{i,u}$ denotes the probability of node $u$ being the initial starting node for $W_i$.
%Let $\Phi(i,k_i) {\defeq} (X_{i,1}, \ldots, X_{i,k_i})$ denote the random variable of the exploration trajectory for $W_i$.
%where its randomness comes from the random exploration as well as the starting distribution $\bm{\alpha}_i$.
The reward for $\Phi(i, k_i)$ is defined as the total weights of \textit{unique} nodes visited by $W_i$, i.e., $\sum_{v \in \bigcup_{j=1}^{k_i}\{X_{i,j}\}}\sigma_v$. 
Considering trajectories of all $W_i$'s, the total reward is the total weights of \textit{unique} nodes visited by all random walkers, i.e., $\sum_{v \in \bigcup_{i=1}^{m}\ \bigcup_{j=1}^{k_i}\{X_{i,j}\}}\sigma_v$.
For notational simplicity, let $\cG {\defeq} (\cG_1, \ldots,
\cG_m)$, $\bm{\alpha} {\defeq} (\bm{\alpha}_1, \ldots, \bm{\alpha}_m)$ and $\bsig=(\sigma_1, ..., \sigma_{|\cV|})$ be the parameters of a problem instance and $\bm{k} {\defeq} (k_1, \ldots, k_m)$ be the allocation vector.
For overlapping multi-layered network $\cG$,
the total expected reward is 
	\begin{equation}\label{eq: over opt}\textstyle
	r_{\cG,\bm{\alpha},\bsig} (\bm{k}) {\defeq} {\E_{\Phi(1,k_1), ..., \Phi(m,k_m)}\left[ \sum_{v \in \bigcup_{i=1}^{m}\ \bigcup_{j=1}^{k_i}\{X_{i,j}\}}\sigma_v \right]},
	\end{equation}
where its explicit formula will be discussed later in Sec.~\ref{sec: equivalent model}.
For non-overlapping $\cG$, 
%there are no overlapping nodes among different layers, i.e., a node can only be visited by the random explorer from the same layer. 
the reward function can be simplified and written as the summation over separated layers, 
	\begin{equation}\label{eq: non-over opt}\textstyle
	r_{\cG,\bm{\alpha},\bsig} (\bm{k}) \defeq {\sum_{i=1}^{m}}{\E_{\Phi(i,k_i)}\left[\sum_{v \in \bigcup_{j=1}^{k_i}\{X_{i,j}\}}\sigma_v \right]}.
	\end{equation}
\noindent\textbf{Problem Formulation.}
We are interested in the \textit{budget allocation problem}: how to allocate the total budget $B \in \Z_{\ge 0}$ to the $m$ explorers so as to maximize the total weights of unique nodes visited. 
Also, we assume there is a budget constraint $\bc \defeq (c_1, ..., c_m)$ such that the allocated budget $k_i$ should not exceed $c_i$, i.e., $k_i \le c_i$, for $i \in [m]$. 
% Without loss of generality, we assume $c_i \le B$ and $\sum_{i=1}^{m}c_i \ge B$.
% otherwise we can safely set $c_i=
%B$ without affecting our analysis and trivially allocate $k_i=c_i$, respectively.
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{-5pt}
\begin{definition}
Given graph structures $\cG \defeq (\cG_1, \ldots,
\cG_m)$, starting distributions $\bm{\alpha}\defeq(\bm{\alpha}_1, \ldots, \bm{\alpha}_m)$, total budget $B$ and budget constraints $\bc \defeq(c_1, ..., c_m)$, the \textbf{Mu}lti-\textbf{La}yered \textbf{N}etwork \textbf{E}xploration problem, denoted as \textbf{\mulane{}}, is formulated as the following optimization problem,
\noindent
\begin{equation}\label{eq: opt budget}
    \text{Maximize} \,\, r_{\cG,\bm{\alpha},\bsig} (\bm{k}) \, s.t. \,\, \bk \in \mathbb{Z}^m_{\ge 0} \le \bc,\, {\sum_{i=1}^{m}}{k_i}\le B,
\end{equation}
% \resizebox{.99\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
% \begin{align}\label{eq: opt budget}\textstyle
% &\quad \quad \quad \quad \quad \text{Maximize} \,\, r_{\cG,\bm{\alpha},\bsig} (\bm{k}) \notag \\ 
% &s.t. \quad {\sum_{i=1}^{m}}{k_i}\le B; \,\, \bk \le \bc;\,\, k_1,\ldots,k_m \in \mathbb{Z}_{\ge 0},
% \end{align}
% \end{minipage}}
\end{definition}
\noindent where $r_{\cG,\bm{\alpha},\bsig} (\bm{k})$ is given by Eq.~(\ref{eq: over opt}) or Eq.~(\ref{eq: non-over opt}).
We also need to consider the following settings:
\setlength{\abovedisplayskip}{7pt}
\setlength{\belowdisplayskip}{7pt}

{\noindent\textbf{\textit{Offline Setting.}} For the offline setting, all problem instance parameters $(\cG, \bm{\alpha}, \bsig, \bc, B)$ are given, and we aim to find the optimal budget
allocation $\bm{k^*}$ determined by Eq.~(\ref{eq:
opt budget}).}
%\item 

\noindent\textbf{\textit{Online Setting.}} 
For the online setting, we consider $T$-round explorations. 
	Before the exploration, we only know an upper bound of the total number of nodes in $\cG$ and
		the number of layers $m$,\footnote{More precisely we only need to know
		the number of independent explorers. 
		If two explorers explore on the same layer, it is equivalent as two layers with identical graph structures.} but we do not know about the network structure $\cG$
		, the starting distributions $\bm{\alpha}$ or node weights $\bsig$.
	In round $t \in [T]$, we choose the budget allocation $\bm{k}_t {\defeq} (k_{t,1}, \ldots, k_{t,m})$ only based on observations from previous rounds, 
		where $k_{t,i}\in \Z_{\ge 0}$ is the budget allocated to the $i$-th layer and $\sum_{i=1}^{m}{k_{t,i}}\le B, \bk_t \le \bc$. 
	Define $\bm{k}_t$ as the {\em action} taken in round $t$. 
	By taking the action $\bm{k}_t$ we mean that we interact with the environment and the random explorer $W_i$, which is part of the environment, would explore $k_{t,i}$ steps and generate
	 the exploration trajectory $\Phi(i, k_{t,i}){=}(X_{i,1}, ..., X_{i,k_{t,i}})$.
% 	Note that the random explorers are considered as part of the environment, not part of our learning algorithm, so they would 
% 		have the knowledge of the graph structure $\cG$ and the starting distribution $\bm{\alpha}$ to properly conduct random
% 		walks on the corresponding layers of the graph.
	{After we take
	the action $\bm{k}_t$, the exploration trajectory $\Phi(i, k_{t,i})$ for each
	layer $L_i$ as well as the fixed importance weight $\sigma_u$ of $u \in \Phi(i,k_{t,i})$ is revealed as the \textit{feedback}\footnote{We further consider random node weights with unknown mean vector $\bsig$, see the \OnlyInFull{Appendix~\ref{appendix: over extend}}\OnlyInShort{supplementary material} for details.}, which  
	we leverage on to
	learn parameters related to the graph structures $\cG$, the starting distribution $\bm{\alpha}$ and the node weights $\bsig$,
		so that we can select better actions in future rounds}.
% \wei{In the online setting, I do not see that an explicit statement saying that the node weight is reveal the first time it is visited.
% 	So I added it above.
% 	I thought about that adding node weight as part of the trajectory, but it seems to be more complicated, so I did not do that.}
The reward we gain in round $t$ is the total weights of unique nodes visited by all random explorers in round $t$.
Our goal is to design an efficient online learning algorithm $A$ to give us guidance on
taking actions and gain as much cumulative reward as possible in $T$ rounds. 

In general, the online
	algorithm has to deal with the exploration-exploitation tradeoff.
	The cumulative~regret is a commonly used metric to evaluate
	the performance of an online learning algorithm $A$.
	%Define $\Phi_t$ as the random variable of exploration trajectory for all communities at time $t$
	{
	Formally, the $T$-round ($(\xi,\beta)$-approximation) regret of $A$ is:
			\begin{equation}\textstyle \label{eq: alpha beta regret}
			Reg_{\cG,\bm{\alpha},\bsig}(T) {=} \xi \beta T\cdot r_{\cG,\bm{\alpha},\bsig}( \bm{k^*}){-}\E\big[ \sum_{t=1}^Tr_{\cG,\bm{\alpha},\sigma}(\bm{k_t}^A)\big],
			%&{=} \alpha\beta T\cdot r_{\cG}(\bm{\alpha}, \bm{k^*}) {-} \mathbb{E}\left\sum_{t=1}^TR\left(\bigcup_{i=1}^{m}\Phi(i,k_{t,i})\right)\right],
			\end{equation} 
			}
	where $r_{\cG,\bm{\alpha},\bsig} (\bm{k^*})$ is the reward value for the optimal budget
	allocation $\bm{k^*}$, $\bm{k}_t^A$ is budget allocation selected by the learning algorithm
	$A$ in round $t$, the expectation is taken over the randomness of the
	algorithm and the exploration trajectories in all $T$ rounds,
	and $(\xi,\beta)$ is the approximation guarantee of the offline oracle as explained below.
Similar to other online learning frameworks~\cite{chen2016combinatorial, wang2017improving}, we assume that the online learning algorithm has access to an offline $(\xi, \beta)$-approximation oracle, which for problem 
instance $(\cG, \bm{\alpha}, \bsig, \bc, B)$ outputs an action $\bk$ such that $\Pr\left(r_{{\cG},\bm{\alpha}, \bsig} (\bk) \ge \xi \cdot r_{{\cG},\bm{\alpha},\bsig}( \bk^*)\right) \ge \beta$.
We also remark that the actual oracle we use takes certain intermediate parameters as inputs instead of $\cG$ and $\bm{\alpha}$.
% We also remark that in our actual online learning algorithms, we do not try to recover the graph structure $\cG$ and the starting distribution $\bm{\alpha}$.
% Instead, we estimate certain intermediate parameters $\bm{\mu}$, and use them together with partial-revealed node weights $\bar{\bsig}$, budget
% 	constraints $B$ and $\bm{c}$ to work with the offline algorithm we designed as the \textit{offline approximation
% 	oracle} for the online learning algorithm.

% \vspace{-5pt}
\textbf{{Submodularity and DR-Submodularity Over Integer lattices.}}
To solve the \mulane{} problem, 
we leverage on the submodular and DR-submodular properties of the reward function.
%Let $\bbR$ and $\bbZ_{\ge 0}$ denote the set of reals and non-negative integers.
For any $\bx, \by \in \bbZ^m_{\ge 0}$, we denote $\bx \vee \by, \bx \wedge \by \in \bbZ^m_{\ge 0} $ as the coordinate-wise maximum and minimum of these two vectors, i.e., $(\bx \vee \by)_i=\max\{x_i, y_i\}, (\bx \wedge \by)_i=\min\{x_i, y_i\}$.
We define a function $f: \bbZ_{\ge 0}^m \rightarrow \bbR$ over the integer lattice $\bbZ^m_{\ge 0 }$ as a \textit{ submodular} function if the following inequality holds for any $\bx, \by \in \bbZ^m_{\ge 0}$:
\begin{equation}\label{ieq: lattice def}\textstyle
f(\bx \vee \by) + f(\bx \wedge \by) \le f(\bx) + f(\by).
\end{equation}
Let $\text{supp}^+(\bx - \by)$ denote the set $I = \{i\in [m]: x_i > y_i\}$,
$\bch_i = (0, ..., 1, ..., 0)$ be the one-hot vector whose $i$-th element is 1 and 0 otherwise, and $\bx \ge \by$ means $x_i \ge y_i$ for all $i \in [m]$.
We define a function $f: \bbZ_{\ge 0}^m \rightarrow \bbR$ as a \textit{DR-submodular} (diminishing return submodular) function if the following inequality holds for any $\bx \le \by$ and $i \in [m]$, 
\begin{equation}\textstyle 
f(\by + \bch_i) - f(\by) \le f(\bx + \bch_i) - f(\bx).
\end{equation}
We say a function $f$ is \textit{monotone} if for any $\bx \le \by$, $f(\bx) \le f(\by)$. 
%Without loss of generality, we assume monotone functions are normalized, i.e., $f(\bm{0})=0$.
Note that for a function $f: \bbZ_{\ge 0}^m \rightarrow \R$, submodularity does not imply DR-submodularity over integer lattices.
In fact, the former is weaker than the latter, that is, a DR-submodular function is always a submodular function, but not vice versa.
However, for a typical submodular function $f: \{0,1\}^m \rightarrow \bbR$ defined on a set, they are equivalent.


==> MuLaNE Camera Ready ICML2021/content/properties.tex <==
%%\vspace{-5pt}
\section{Equivalent Bipartite Coverage Model}\label{sec: equivalent model}
In order to derive the explicit formulation of the reward function $r_{\cG, \bm{\alpha},\bsig}( \bk)$ in Eq.~(\ref{eq: over opt}),
we construct an undirected bipartite coverage graph $\cB(\cW,\cV,\cE')$, where $\cW=\{W_1, ..., W_m\}$ denotes $m$ random explorers,
$\cV=\bigcup_{i \in [m]}{\cV_i}$ denotes all possible distinct nodes to be explored in $\cG$, and the edge set $\cE'{=}\{(W_i,u)|u \in \cV_i, i \in [m]\}$ indicating whether node $u$ could be visited by $W_i$. 
For each edge $(W_i, u) \in \cE'$, we associate it with $c_i+1$ visiting probabilities denoted as $P_{i,u}(k_i)$ for $k_i \in \{0\} \cup  [c_i]$.
$P_{i,u}(k_i)$ represents the probability that the node $u$ is visited by the random walker $W_i$ given the budget $k_i$, i.e., $P_{i,u}(k_i)=\Pr(u \in \Phi(i,k_i))$.
Since $W_i$ can never visit the node outside the $i$-th layer (i.e., $u \notin \cG_i$), we set $P_{i,u}(k_i)=0$ if $(W_i, u) \not\in \cE'$. 
Then, given budget allocation $\bk$, the probability of a node $u$ visited by at least one random explorer is $\Pr(u, \bk){=} 1-\Pi_{i\in[m]}(1-P_{i,u}(k_i))$ because each $W_i$ has the independent probability $P_{i,u}(k_i)$ to visit $u$. 

By summing over all possible nodes, the reward function is 
\begin{equation}\label{eq: over reward}\textstyle
r_{\cG,\bm{\alpha}, \bsig}(\bm{k})=\sum_{u\in\cV}\sigma_u\left(1-\Pi_{i\in[m]}\left(1-P_{i,u}(k_i)\right)\right)
\end{equation}
According to Eq.~(\ref{eq: non-over opt}), for non-overlapping multi-layered network, we can rewrite the reward function as:
\begin{equation}\label{eq: non-over reward}\textstyle
    r_{\cG,\bm{\alpha},\bsig} (\bm{k})=\sum_{i\in[m]}\sum_{u \in \cV_i}\sigma_u P_{i,u}(k_i).
\end{equation}

\noindent\textbf{Remark.}
The bipartite coverage model is needed to integrate the graph structure and the random walk exploration mechanisms into $P_{i,u}(k_i)$ to determine the reward function. It also handles the scenario where each layer is explored by multiple random walkers \OnlyInFull{(see Appendix~\ref{appendix: multiple})}\OnlyInShort{(see supplementary material)}. 
% Without loss of generality, suppose we want to add a new random walker $W_1'$ to the layer $L_1$. 
% A new node $W_1'$ can be easily added to $\cL$ representing the new random explorer, and new edges $\{(W_1', u)|u \in \cV_1\}$ are added to $\cE'$. 
% Thus, we can use the same algorithms and analysis to solve the optimization problem on the newly constructed bipartite coverage graph.

%\section{Deriving Explicit Formula of the Visiting Probability $P_{i,u}(k_i)$ and Its Properties}\label{sec: explicit formula}
\subsection{Properties of the visiting probability $P_{i,u}(k_i)$}\label{sec: explicit formula}

The quantities $P_{i,u}(k_i)$'s in Eq.~\eqref{eq: over reward} and~\eqref{eq: non-over reward} are crucial for both our
	offline and online algorithms, and thus we provide their analytical formulas and properties here.
In order to analyze the property of the reward function, we apply the absorbing Markov Chain technique to calculate $P_{i,u}(k_i)$.
For $u \notin \cG_i$, $P_{i,u}(k_i)=0$;
For $u \in \cG_i$, we create an absorbing Markov Chain $\bm{P_i(u)} \in \R^{n_i \times n_i}$ by setting the target node $u$ as the absorbing node. 
We derive the corresponding transition matrix $\bm{P_i(u)}$ as 
$\bm{P_i(u)}[v,\cdot] = \bch_u^{\top}$ if $v$ = $u$ and $\bm{P_i(u)}[v,\cdot]
=\bm{P_i}{[v,\cdot]}$ otherwise,
where $\bm{P_i}{[v,\cdot]}$ denotes the row vector corresponding to the node $v$ of $\bm{P_i}$,
 and $\bch_u= (0, ..., 0, 1, 0, ..., 0 )^\top$ denotes the one-hot vector with $1$ at the $u$-th entry and $0$ 
 elsewhere.\footnote{When related to matrix operations, we treat all vectors as column vectors by default.}
Intuitively, $\bm{P_i(u)}$ corresponds to the transition probability matrix of $\cG_i$ after removing all out-edges of $u$ and adding a self loop to itself in the original graph $\cG_i$. 
The random walker $W_i$ will be trapped in $u$ if it ever visits $u$.
We observe that $P_{i,u}(k_i)$ equals to the probability the random walker stays in
the absorbing node $u$ at step $k_i \in \bbZ_{> 0}$ (trivially, $P_{i,u}(0)=0
$), %if it starts from the initial distribution $\bm{\alpha_i}$, i.e.,
\begin{equation}\label{eq: simple form}\textstyle
P_{i,u}(k_i)=\bm{\alpha_i}^{\top} \bm{P_i(u)}^{k_i-1} \bch_u.
\end{equation}
%To see this, the probability that node $u$ has not been visited before (included) step $k$ equals to $\bm{\alpha} \bm{P}(u)^{k-1}(\bm{1}-\bch_u)$, where $\bm{1} \in \R^{1\times n}$ is the all 1 vector. From this, we have $1-\Pr(u,k)= 1-\bm{\alpha} \bm{P}(u)^{k-1} \bch_u$. 
Then define the marginal gain of $P_{i,u}(\cdot)$ at step $k_i\ge1$ as,
\begin{equation}\label{eq: marginal gain}\textstyle
g_{i,u}(k_i) = P_{i,u}(k_i) - P_{i,u}(k_i-1).
\end{equation}
The physical meaning of $g_{i,u}(k_i)$ is the probability that node $u$ is visited exactly at the $k_i$-th step and not visited before $k_i$. 
Now, we can show $g_{i,u}(k_i)$ is non-negative,
\begin{restatable}{lemma}{lemNonDecreasing}\label{lem: non-decreasing}
$g_{i,u}(k_i) \ge 0$ for any $i\in [m]$, $u \in \cV_i$, $k_i\in \Z_{> 0}$.
\end{restatable}
This means
$P_{i,u}(k_i)$ is non-decreasing with respect to step $k_i$.
In other words, the more budgets we allocate to $W_i$, the higher probability $W_i$ can visit $u$ in $k_i$ steps. 


\noindent{\textbf{Starting from arbitrary distributions:}}
Although $P_{i,u}(k_i)$ is monotone (non-decreasing) w.r.t $k_i$, 
 $g_{i,u}(k_i)$ may not be monotonic non-increasing under arbitrary staring distributions.
Intuitively, there may exist one critical step $k_i$ such that $P_{i,u}(k_i)$ suddenly increases by a large value \OnlyInFull{(see Appendix~\ref{appendix: explct form stationary})}\OnlyInShort{(see supplementary material)}.
%This is counter intuitive because
%For example, consider a path $P_3$ with three nodes as the $i$-th layer $\cG_i(\cV_i, \cE_i)$, where $\cV_i=\{u,v,w\}$ and $\cE_i=\{(u,v),(v,u), (v,w), (w,v)\}$. If the $W_i$ always starts from the left-most node $u$ and chooses the right-most node $w$ as our target node. Then, $g_{i,w}(1)=g_{i,w}(2)=0$ but $g_{i,w}(3)>0$ since at least three steps are needed to visit the node $w$, which shows that $g_{i,w}(k_i)$ is not always non-increasing.
This means that $P_{i,u}(k_i)$ lacks the diminishing return (or ``discretely concave") property, which many problems rely on to provide good optimization~\cite{kapralov2013online,soma2015generalization}.
In other words, we are dealing with a more challenging non-concave optimization problem for the discrete budget allocation.

\noindent{\textbf{Starting from the stationary distribution:}}
If our walkers start with the stationary distributions, the following property holds: $g_{i,u}(k_i)$ is non-increasing w.r.t $k_i$.
\begin{restatable}{lemma}{thmStationary}\label{lem: stationary}
	$g_{i,u}(k_i+1) - g_{i,u}(k_i) \le 0$ for any $i\in [m]$, $u \in \cV_i$, $k_i\in \Z_{> 0}$, if $\bm{\alpha}_i=\bm{\pi_i}$, where $\bm{\pi_i}^{\top}\bm{P_i}=\bm{\pi_i}^{\top}$.
\end{restatable}

% % omit
% \xutong{
% More interestingly, the stationary distribution $\bm{\pi}_i$ is the \textit{only} starting distribution for $\bP_i$ such that for any $u \in \cV_i, k_i \in \Z_{>0}$, $g_{i,u}(k_i+1) - g_{i,u}(k_i) \le 0$ when $\bP_i$ is ergodic (the random walker can visit any node in finite steps starting from any node) and there are no self loops (the random walker will not stay in the same node in any two consecutive steps) in $\cG_i$.
% This means that the diminishing return property is missing for most starting distributions.
% \OnlyInShort{See the supplementary material for details.}
% \OnlyInFull{The proofs are included in the Appendix~\ref{appendix: explct form}.}
% }


==> MuLaNE Camera Ready ICML2021/content/related.tex <==
\vspace{-9pt}
\subsection{Related Work}\label{sec: related work}
\vspace{-5pt}
%\textbf{Related Work}
Network exploration via random walks has been studied in various application contexts such as community detection~\cite{pons2005computing}, centrality measuring~\cite{gleich2015pagerank},
	large-scale network sampling~\cite{li2019walking}, and influence maximization~\cite{wilder2018maximizing}.
Multiple random walks has also been used, e.g. in~\cite{lv2002search} for query resolution in peer-to-peer networks.
However, none of these studies address the budgeted MuLaNE problem.
% (I think this part can be removed if we have no space.)
\mulane{} is also related to the influence maximization (IM) problem~\cite{kempe2003maximizing, chen2009efficient} and can be viewed as a special variant of IM. 
Different from the standard Independent Cascade (IC) model~\cite{wang2012scalable} in IM, which randomly broadcasts to all its neighbors, the propagation process of \mulane{} is a random walk that selects one neighbor. Moreover, each unit of budget in \mulane{} is used to propagate one random-walk step, not to select one seed node as in IC. 

The offline budget allocation problem has been studied by \citet{alon2012optimizing,soma2014optimal}, the latter of which
propose the lattice submodularity and a constant approximation algorithm based on this property.
Our offline overlapping MuLaNE setting is based on a similar approach, but we provide a better approximation ratio compared to the original analysis in~\cite{alon2012optimizing}.
Moreover, we further show that the stationary setting enjoys DR-submodularity, leading to an efficient algorithm with a better approximation ratio.


The multi-armed bandit (MAB) problem is first studied by \citet{robbins1952some} and then extended by many studies
(cf. \cite{BCB12}).
Our online MuLaNE setting fits into the general Combinatorial MAB (CMAB) framework of~\cite{gai2012combinatorial,chen2016combinatorial}.
CUCB is proposed as a general algorithm for CMAB~\cite{chen2016combinatorial}.
Our study includes several adaptations, such as handling unknown node weights, defining intermediate random variables as base arms and so on.


\citet{chen2018community} study the community exploration problem, which is essentially a special case of MuLaNE with
	non-overlapping complete graphs.
As a result, their technique is different and much simpler than ours. 

The rest of the paper is organized as follows. 
Section \ref{sec: problem setting} states the settings of \mulane;
Section \ref{sec: equivalent model} states the equivalent bipartite coverage model to derive the explicit form for our reward function;
Section \ref{sec: offline opt} states offline algorithms for four offline settings with provable approximation guarantee and running time analysis;
Section \ref{sec: online learning} states two online learning algorithms with regret analysis;
Empirical results are shown in Section \ref{sec: experiments};
and Section \ref{sec: conclusion} concludes the paper.


